Syzygy: Dual Code-Test C to (safe) Rust Translation using LLMs and Dynamic Analysis

Despite extensive usage in high-performance, low-level systems programming applications, C is susceptible to vulnerabilities due to manual memory management and unsafe pointer operations. Rust, a modern systems programming language, offers a compelling alternative. Its unique ownership model and type system ensure memory safety without sacrificing performance. In this paper, we present Syzygy, an automated approach to translate C to safe Rust. Our technique uses a synergistic combination of LLM-driven code and test translation guided by dynamic-analysis-generated execution information. This paired translation runs incrementally in a loop over the program in dependency order of the code elements while maintaining per-step correctness. Our approach exposes novel insights on combining the strengths of LLMs and dynamic analysis in the context of scaling and combining code generation with testing. We apply our approach to successfully translate Zopfli, a high-performance compression library with ~3000 lines of code and 98 functions. We validate the translation by testing equivalence with the source C program on a set of inputs. To our knowledge, this is the largest automated and test-validated C to safe Rust code translation achieved so far.

==> sta-_STALE_.tex <==
\subsection{Semantic Type Alignment}
\label{subsec:semtypealign}


% \ms{should we fold this into Section \ref{subsec:argtrans}?}
% \ag{there is a dependency with codegen as well though, I think? (the type translation is also relevant as a feasibility concern). I agree that perhaps a separate section is not warranted, it is a bit weird}
% \ms{ah I see, separate section is fine; what's unclear to me is distinction, if any, between the module \semtypealigner{} (generating \rustc{translate\_args}) and this sec. (which prolly highlights challenges and only affects codegen prompts).}

Translation between imperative typed languages can be conceptually thought of a combination of two operations: (1) converting/lifting types of variables, and (2) translating expressions and statements on these variables.
% 
% The choice of type lifts (1) affects/restricts the operations one can perform in (2).
% 
This is particularly important for our FAT approach operates by creating semantically \textit{similar} functions in Rust.
% 

The key challenge here arises due to pointers in C. This is because, \textit{pointers hide information regarding the underlying object structure, and how its used.}
% 
(Safe) Rust does not allow C-like pointers, thus \textit{translation needs to recover this hidden information}.
% 
In addition to all of these void pointers in C further obfuscate information by also hiding the type of the underlying object.
%
We now discuss this challenge further through the following table.

\begin{table}[h]
    \centering
    \begin{tabular}{c | c | c}
        \hline
        Scenario & C type & Possible Rust type
        \\ \hline 
        Array pointer & \cct{(T *)} & \rustct{Vec<T>}, \rustct{[T; N]} \\
        Singleton pointer immutable & \cct{(T *)} & \rustct{& T} \\
        Singleton pointer mutable & \cct{(T *)} & \rustct{&mut T}, \rustct{RefCell<T>}, \rustct{Rc<RefCell<T>>} \\ \hline
        Standard objects (e.g., strings) & \cct{(char *)} & \rustct{crate::string} \\ \hline
    \end{tabular}
    \caption{\nj{can pass by value also i think}}
\end{table}
% 

\Paragraph{Pointers hide object structure}
% 
A C pointer can be used for a singleton object as well as arrays. The target corresponding Rust type may vary between these cases.
% 
Further C does not have standard library objects (e.g., strings), rather these are just represented as \cc{char}/\cc{uchar} arrays. 


\Paragraph{Pointers hide usage information}
% 
For example, if argument \cc{a} in function \cc{f} (Fig. \ref{fig:example}) was aliased with a pointer from an outer scope, the Rust version of \cc{f} would have to make sure that the shared object (and not a copy) was modified.
% 
Although this is easier in C due to full control over reads/writes with pointers, Rust imposes strict borrowing and mutability rules that must be followed: (\rustc{&}, \rustc{&mut}, \rustc{RefCell<T>}, \rustc{Rc<RefCell<T>>}).
% 
In addition to type universality, C pointers enable arbitrary reads and writes, which is not the case in Rust. In Rust, we need to specify mutability and non-nullability, as well as carefully manage aliases between pointers \adwaittodo{say something smart about the borrowing model in Rust}.
